Measuring In-Context Computation Complexity via Hidden State Prediction

Detecting when a neural sequence model does "interesting" computation is an open problem. The next token prediction loss is a poor indicator: Low loss can stem from trivially predictable sequences that are uninteresting, while high loss may reflect unpredictable but also irrelevant information that can be ignored by the model. We propose a better metric: measuring the model's ability to predict its own future hidden states. We show empirically that this metric -- in contrast to the next token prediction loss -- correlates with the intuitive interestingness of the task. To measure predictability, we introduce the architecture-agnostic "prediction of hidden states" (PHi) layer that serves as an information bottleneck on the main pathway of the network (e.g., the residual stream in Transformers). We propose a novel learned predictive prior that enables us to measure the novel information gained in each computation step, which serves as our metric. We show empirically that our metric predicts the description length of formal languages learned in-context, the complexity of mathematical reasoning problems, and the correctness of self-generated reasoning chains.

==> biblio_old.tex <==
NLP:
@STRING{confEMNLP={Proc. Conf. on Empirical Methods in Natural Language Processing (EMNLP)}}
@STRING{confNAACL = "Proc. North American Chapter of the Association for Computational Linguistics on Human Language Technologies (NAACL-HLT)"}
@STRING{confACL = "Proc. Association for Computational Linguistics (ACL)"}
@STRING{TACL = "Transactions of the Association for Computational Linguistics (TACL)"}
@STRING{confACLIJCNLP = "Proc. of Annual Meeting of the Association for Computational
               Linguistics and the International Joint Conf. on Natural
               Language Processing, {ACL-IJCNLP}"}

Machine Learning:
@STRING{confICLR = "Int. Conf. on Learning Representations (ICLR)"}
@STRING{confICLRW = "Int. Conf. on Learning Representations (ICLR), Workshop"}
@STRING{confNIPS = "Proc. Advances in Neural Information Processing Systems (NIPS)"}
@STRING{confNEU = "Proc. Advances in Neural Information Processing Systems (NeurIPS)"}
@STRING{confICML = "Proc. Int. Conf. on Machine Learning (ICML)"}
@STRING{confAAAI = "Proc. {AAAI} Conf. on Artificial Intelligence"}
@STRING{confICANN = "Proc. Int. Conf. on Artificial Neural Networks (ICANN)"}
@STRING{confAISTATS = "Proc. Int. Conf. on Artificial Intelligence and Statistics (AISTATS)"}

@STRING{IJPRAI = "Int. Journal of Pattern Recognition and Artificial Intelligence (IJPRAI)"}
@STRING{confJMLR = "Journal of Machine Learning Research (JMLR)"}


Vision:
@STRING{confCVPR = "Proc. The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)"}
@STRING{confECCV = "Proc. European Conference on Computer Vision (ECCV)"}
@STRING{confICCV = "Proc. IEEE Int. Conf. on Computer Vision (ICCV)"}

Other:
@STRING{confICASSP = "Proc. {IEEE} Int. Conf. on Acoustics, Speech and Signal Processing (ICASSP)"}

@STRING{confALIFE = "Proc. Int. Conf. on the Simulation and Synthesis of Living Systems (ALIFE)"}

@inproceedings{Storck:95,
author = {J. Storck and S. Hochreiter and J. Schmidhuber},
title =  {Reinforcement driven information acquisition in non-deterministic
environments},
booktitle = {Proceedings of the International Conference on
Artificial Neural Networks, Paris},
publisher = {EC2 \& Cie},
volume={2},
pages = {159-164},
year   = {1995}}

@incollection{itti:05,
 title = {Bayesian Surprise Attracts Human Attention},
 author = {L. Itti and P. F. Baldi},
 booktitle = {Advances in Neural Information Processing Systems  (NIPS) 19},
 publisher = {MIT Press},
 address = {Cambridge, MA},
 pages = {547--554},
 year = {2005}
}

@article{Graves2014NeuralTM,
  title={Neural Turing Machines},
  author={Alex Graves and Greg Wayne and Ivo Danihelka},
  journal={ArXiv},
  year={2014},
  volume={abs/1410.5401},
}

@inproceedings{herrmann2023learning,
  title={Learning one abstract bit at a time through self-invented experiments encoded as neural networks},
  author={Herrmann, Vincent and Kirsch, Louis and Schmidhuber, J{\"u}rgen},
  booktitle={International Workshop on Active Inference},
  pages={254--274},
  year={2023},
  organization={Springer}
}

@article{Kirsch2022GeneralPurposeIL,
  title={General-Purpose In-Context Learning by Meta-Learning Transformers},
  author={Louis Kirsch and James Harrison and Jascha Narain Sohl-Dickstein and Luke Metz},
  journal={ArXiv},
  year={2022},
  volume={abs/2212.04458},
}

@InProceedings{lehmann:08,
  author = "J. Lehman and K. O. Stanley",
  title = "Exploiting open-endedness to solve problems through the search for novelty",
  booktitle = "Proc. Eleventh International Conference on Artificial Life (ALIFE XI), Cambridge, MA",
  year = 2008
}


@InProceedings{pmlr-v235-hughes24a,
  title = 	 {Position: Open-Endedness is Essential for Artificial Superhuman Intelligence},
  author =       {Hughes, Edward and Dennis, Michael D and Parker-Holder, Jack and Behbahani, Feryal and Mavalankar, Aditi and Shi, Yuge and Schaul, Tom and Rockt\"{a}schel, Tim},
  booktitle = 	 {Proceedings of the 41st International Conference on Machine Learning},
  pages = 	 {20597--20616},
  year = 	 {2024},
  volume = 	 {235},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {21--27 Jul},
  publisher =    {PMLR},
}

@article{deletang2023compression,
  author       = {Gr{\'{e}}goire Del{\'{e}}tang and
                  Anian Ruoss and
                  Paul{-}Ambroise Duquenne and
                  Elliot Catt and
                  Tim Genewein and
                  Christopher Mattern and
                  Jordi Grau{-}Moya and
                  Li Kevin Wenliang and
                  Matthew Aitchison and
                  Laurent Orseau and
                  Marcus Hutter and
                  Joel Veness},
  title        = {Language Modeling Is Compression},
  journal      = {CoRR},
  volume       = {abs/2309.10668},
  year         = {2023},
  eprinttype    = {arXiv},
  eprint       = {2309.10668},
  timestamp    = {Mon, 25 Sep 2023 15:34:00 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2309-10668.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{olsson2022context,
   title={In-context Learning and Induction Heads},
   author={Olsson, Catherine and Elhage, Nelson and Nanda, Neel and Joseph, Nicholas and DasSarma, Nova and Henighan, Tom and Mann, Ben and Askell, Amanda and Bai, Yuntao and Chen, Anna and Conerly, Tom and Drain, Dawn and Ganguli, Deep and Hatfield-Dodds, Zac and Hernandez, Danny and Johnston, Scott and Jones, Andy and Kernion, Jackson and Lovitt, Liane and Ndousse, Kamal and Amodei, Dario and Brown, Tom and Clark, Jack and Kaplan, Jared and McCandlish, Sam and Olah, Chris},
   year={2022},
   journal={Transformer Circuits Thread},
   note={https://transformer-circuits.pub/2022/in-context-learning-and-induction-heads/index.html}
}

@inproceedings{gpt3,
  title={Language models are few-shot learners},
  author={Brown, Tom B and others},
  booktitle=confNEU,
  address = {Virtual only},
  month = dec,
  year={2020}
}

@article{elman1990rnn,
  author    = {Jeffrey L. Elman},
  title     = {Finding Structure in Time},
  journal   = {Cognitive Science},
  volume    = {14},
  number    = {2},
  pages     = {179--211},
  year      = {1990}
}


@incollection{jordan1986,
  title={Attractor dynamics and parallelism in a connectionist sequential machine},
  author={Jordan, Michael I},
  booktitle={Proc. Conf. of the Cognitive Science Society},
  address = {Amherst, MA, USA},
  month = aug,
  pages = {531--546},
  year={1986}
}


@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  year={1997},
  pages={1735--1780}
}

@inproceedings{menon2022forget,
  title={Forget-me-not! contrastive critics for mitigating posterior collapse},
  author={Menon, Sachit and Blei, David and Vondrick, Carl},
  booktitle={Uncertainty in Artificial Intelligence},
  pages={1360--1370},
  year={2022},
  organization={PMLR}
}

@inproceedings{Oord2017NeuralDR,
  title={Neural Discrete Representation Learning},
  author={A{\"a}ron van den Oord and Oriol Vinyals and Koray Kavukcuoglu},
  booktitle={Neural Information Processing Systems},
  year={2017},
}

@article{Schmidhuber:92ncfastweights,
author = {J\"urgen Schmidhuber},
title =  { Learning to Control Fast-Weight Memories: An Alternative to
Recurrent Nets},
journal={Neural Computation},
volume = {4},
number = {1},
pages={131-139},
year   = {1992}}

@inproceedings{vaswani2017attention,
  author    = {Ashish Vaswani and
               Noam Shazeer and
               Niki Parmar and
               Jakob Uszkoreit and
               Llion Jones and
               Aidan N. Gomez and
               Lukasz Kaiser and
               Illia Polosukhin},
  title     = {Attention is All you Need},
  booktitle = confNIPS,
  year      = {2017},
  pages     = {5998--6008},
  address   = "Long Beach, CA, USA",
  month = {December}
}

@inproceedings{zhao2021calibrate,
  author       = {Zihao Zhao and
                  Eric Wallace and
                  Shi Feng and
                  Dan Klein and
                  Sameer Singh},
  title        = {Calibrate Before Use: Improving Few-shot Performance of Language Models},
booktitle = confICML,
month = {July},
address = {Virtual only},
  volume       = {139},
  pages        = {12697--12706},
  year         = {2021},
}

@inproceedings{liu2022what,
  author       = {Jiachang Liu and
                  Dinghan Shen and
                  Yizhe Zhang and
                  Bill Dolan and
                  Lawrence Carin and
                  Weizhu Chen},
  title        = {What Makes Good In-Context Examples for GPT-3?},
  booktitle    = {Deep Learning Inside Out Workshop at ACL},
location={Dublin, Ireland},
month={May},
year={2022},
}

@inproceedings{akyurek2024incontext,
  author       = {Ekin Aky{\"{u}}rek and
                  Bailin Wang and
                  Yoon Kim and
                  Jacob Andreas},
  title        = {In-Context Language Learning: Architectures and Algorithms},
  booktitle    = confICML,
address={Vienna, Austria},
month={July},
  year         = {2024},
}

@inproceedings{wei2022cot,
  author       = {Jason Wei and
                  Xuezhi Wang and
                  Dale Schuurmans and
                  Maarten Bosma and
                  Brian Ichter and
                  Fei Xia and
                  Ed H. Chi and
                  Quoc V. Le and
                  Denny Zhou},
  title        = {Chain-of-Thought Prompting Elicits Reasoning in Large Language Models},
  booktitle    = confNEU,
address={New Orleans,
                  LA, USA},
month={November},
  year         = {2022},
}


@inproceedings{lewkowycz2022solving,
  author       = {Aitor Lewkowycz and
                  Anders Andreassen and
                  David Dohan and
                  Ethan Dyer and
                  Henryk Michalewski and
                  Vinay V. Ramasesh and
                  Ambrose Slone and
                  Cem Anil and
                  Imanol Schlag and
                  Theo Gutman{-}Solo and
                  Yuhuai Wu and
                  Behnam Neyshabur and
                  Guy Gur{-}Ari and
                  Vedant Misra},
  title        = {Solving Quantitative Reasoning Problems with Language Models},
    booktitle    = confNEU,
address={New Orleans,
                  LA, USA},
month={November},
  year         = {2022},
}

@inproceedings{zelikman2022star,
  author       = {Eric Zelikman and
                  Yuhuai Wu and
                  Jesse Mu and
                  Noah D. Goodman},
  title        = {STaR: Bootstrapping Reasoning With Reasoning},
      booktitle    = confNEU,
address={New Orleans,
                  LA, USA},
month={November},
  year         = {2022},
}

@inproceedings{kingma2014autoecoder,
  author       = {Diederik P. Kingma and
                  Max Welling},
  editor       = {Yoshua Bengio and
                  Yann LeCun},
  title        = {Auto-Encoding Variational Bayes},
  booktitle    = confICLR,
address={Banff, AB, Canada},
month={April},
  year         = {2014},
}


@inproceedings{rezende2014stochastic,
  author       = {Danilo Jimenez Rezende and
                  Shakir Mohamed and
                  Daan Wierstra},
  title        = {Stochastic Backpropagation and Approximate Inference in Deep Generative
                  Models},
  booktitle    = confICML, address={Beijing, China}, month={June},
  volume       = {32},
  pages        = {1278--1286},
  year         = {2014},
}


@article{dubey2024llama,
  author       = {Abhimanyu Dubey and
                  Abhinav Jauhri and
                  Abhinav Pandey and
                  Abhishek Kadian and
                  Ahmad Al{-}Dahle and
                  Aiesha Letman and
                  Akhil Mathur and
                  Alan Schelten and
                  Amy Yang and
                  Angela Fan and
                  Anirudh Goyal and
                  Anthony Hartshorn and
                  Aobo Yang and
                  Archi Mitra and
                  Archie Sravankumar and
                  Artem Korenev and
                  Arthur Hinsvark and
                  Arun Rao and
                  Aston Zhang and
                  Aur{\'{e}}lien Rodriguez and
                  Austen Gregerson and
                  Ava Spataru and
                  Baptiste Rozi{\`{e}}re and
                  Bethany Biron and
                  Binh Tang and
                  Bobbie Chern and
                  Charlotte Caucheteux and
                  Chaya Nayak and
                  Chloe Bi and
                  Chris Marra and
                  Chris McConnell and
                  Christian Keller and
                  Christophe Touret and
                  Chunyang Wu and
                  Corinne Wong and
                  Cristian Canton Ferrer and
                  Cyrus Nikolaidis and
                  Damien Allonsius and
                  Daniel Song and
                  Danielle Pintz and
                  Danny Livshits and
                  David Esiobu and
                  Dhruv Choudhary and
                  Dhruv Mahajan and
                  Diego Garcia{-}Olano and
                  Diego Perino and
                  Dieuwke Hupkes and
                  Egor Lakomkin and
                  Ehab AlBadawy and
                  Elina Lobanova and
                  Emily Dinan and
                  Eric Michael Smith and
                  Filip Radenovic and
                  Frank Zhang and
                  Gabriel Synnaeve and
                  Gabrielle Lee and
                  Georgia Lewis Anderson and
                  Graeme Nail and
                  Gr{\'{e}}goire Mialon and
                  Guan Pang and
                  Guillem Cucurell and
                  Hailey Nguyen and
                  Hannah Korevaar and
                  Hu Xu and
                  Hugo Touvron and
                  Iliyan Zarov and
                  Imanol Arrieta Ibarra and
                  Isabel M. Kloumann and
                  Ishan Misra and
                  Ivan Evtimov and
                  Jade Copet and
                  Jaewon Lee and
                  Jan Geffert and
                  Jana Vranes and
                  Jason Park and
                  Jay Mahadeokar and
                  Jeet Shah and
                  Jelmer van der Linde and
                  Jennifer Billock and
                  Jenny Hong and
                  Jenya Lee and
                  Jeremy Fu and
                  Jianfeng Chi and
                  Jianyu Huang and
                  Jiawen Liu and
                  Jie Wang and
                  Jiecao Yu and
                  Joanna Bitton and
                  Joe Spisak and
                  Jongsoo Park and
                  Joseph Rocca and
                  Joshua Johnstun and
                  Joshua Saxe and
                  Junteng Jia and
                  Kalyan Vasuden Alwala and
                  Kartikeya Upasani and
                  Kate Plawiak and
                  Ke Li and
                  Kenneth Heafield and
                  Kevin Stone and
                  et al.},
  title        = {The Llama 3 Herd of Models},
  journal   = {Preprint arXiv:2407.21783},
  year         = {2024},
}

@inproceedings{blier2018description,
  author       = {L{\'{e}}onard Blier and
                  Yann Ollivier},
  title        = {The Description Length of Deep Learning models},
  booktitle    = confNEU,
month = {December},
address = {Montr{\'{e}}al, Canada},
  pages        = {2220--2230},
  year         = {2018},
}

@article{elmoznino2024incontext,
  author       = {Eric Elmoznino and
                  Tom Marty and
                  Tejas Kasetty and
                  L{\'{e}}o Gagnon and
                  Sarthak Mittal and
                  Mahan Fathi and
                  Dhanya Sridhar and
                  Guillaume Lajoie},
  title        = {In-context learning and Occam's razor},
  journal   = {Preprint arXiv:2410.14086},
  year         = {2024},
}

@inproceedings{jiang2020inserting,
  author       = {Zhiying Jiang and
                  Raphael Tang and
                  Ji Xin and
                  Jimmy Lin},
  title        = {Inserting Information Bottlenecks for Attribution in Transformers},
booktitle   = confEMNLP,
  year         = {2020},
address = {Virtual only},
month={November}
}

@inproceedings{devlin2019bert,
  author       = {Jacob Devlin and
                  Ming{-}Wei Chang and
                  Kenton Lee and
                  Kristina Toutanova},
  title        = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
                  Understanding},
  booktitle    = confNAACL,
address={Minneapolis, MN, USA},
month={June},
  pages        = {4171--4186},
  year         = {2019},
}


@article{bricken2023monosemanticity,
       title={Towards Monosemanticity: Decomposing Language Models With Dictionary Learning},
       author={Bricken, Trenton and Templeton, Adly and Batson, Joshua and Chen, Brian and Jermyn, Adam and Conerly, Tom and Turner, Nick and Anil, Cem and Denison, Carson and Askell, Amanda and Lasenby, Robert and Wu, Yifan and Kravec, Shauna and Schiefer, Nicholas and Maxwell, Tim and Joseph, Nicholas and Hatfield-Dodds, Zac and Tamkin, Alex and Nguyen, Karina and McLean, Brayden and Burke, Josiah E and Hume, Tristan and Carter, Shan and Henighan, Tom and Olah, Christopher},
       year={2023},
       journal={Transformer Circuits Thread},
       note={https://transformer-circuits.pub/2023/monosemantic-features/index.html}
    }

@article{elhage2022superposition,
   title={Toy Models of Superposition},
   author={Elhage, Nelson and Hume, Tristan and Olsson, Catherine and Schiefer, Nicholas and Henighan, Tom and Kravec, Shauna and Hatfield-Dodds, Zac and Lasenby, Robert and Drain, Dawn and Chen, Carol and Grosse, Roger and McCandlish, Sam and Kaplan, Jared and Amodei, Dario and Wattenberg, Martin and Olah, Christopher},
   year={2022},
   journal={Transformer Circuits Thread},
   note={https://transformer-circuits.pub/2022/toy\_model/index.html}
}

@inproceedings{henderson2023vae,
  author       = {James Henderson and
                  Fabio Fehr},
  title        = {A {VAE} for Transformers with Nonparametric Variational Information
                  Bottleneck},
  booktitle    = confICLR,
address={Kigali, Rwanda},
month={May},
  year         = {2023},
}


@inproceedings{bahdanau2015neural,
  author    = {Dzmitry Bahdanau and
               Kyunghyun Cho and
               Yoshua Bengio},
  title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
  booktitle = confICLR,
  year      = {2015},
  address   = {San Diego, CA, USA},
  month     = {May},
}

@inproceedings{hendrycks2021math,
  author       = {Dan Hendrycks and
                  Collin Burns and
                  Saurav Kadavath and
                  Akul Arora and
                  Steven Basart and
                  Eric Tang and
                  Dawn Song and
                  Jacob Steinhardt},
  editor       = {Joaquin Vanschoren and
                  Sai{-}Kit Yeung},
  title        = {Measuring Mathematical Problem Solving With the {MATH} Dataset},
  booktitle    =confNEU,
month={December},
  year         = {2021},
}

@article{cobbe2021training,
  author       = {Karl Cobbe and
                  Vineet Kosaraju and
                  Mohammad Bavarian and
                  Mark Chen and
                  Heewoo Jun and
                  Lukasz Kaiser and
                  Matthias Plappert and
                  Jerry Tworek and
                  Jacob Hilton and
                  Reiichiro Nakano and
                  Christopher Hesse and
                  John Schulman},
  title        = {Training Verifiers to Solve Math Word Problems},
journal   = {Preprint arXiv:2110.14168},
  year         = {2021},
}

@article{Schmidhuber1992LearningCE,
  author = {Schmidhuber, J{\"u}rgen},
  title = {Learning Complex, Extended Sequences Using the Principle of History Compression},
  journal = {Neural Computation},
  volume = {4},
  pages = {234--242},
  year = {1992},
}

@article{Schmidhuber1993DiscoveringPC,
  author = {J{\"u}rgen Schmidhuber and Daniel Prelinger},
  title = {Discovering Predictable Classifications},
  journal = {Neural Computation},
  volume = {5},
  pages = {625--635},
  year = {1993},
}

@article{Guo2020BootstrapLR,
  author = {Zhaohan Daniel Guo and Bernardo {'A}vila Pires and Bilal Piot and Jean-Bastien Grill and Florent Altch{'e} and R{'e}mi Munos and Mohammad Gheshlaghi Azar},
  title = {Bootstrap Latent-Predictive Representations for Multitask Reinforcement Learning},
  journal = {ArXiv},
  volume = {abs/2004.14646},
  year = {2020},
}

@inproceedings{Schwarzer2020DataEfficientRL,
  author = {Max Schwarzer and Ankesh Anand and Rishab Goel and R. Devon Hjelm and Aaron C. Courville and Philip Bachman},
  title = {Data-Efficient Reinforcement Learning with Self-Predictive Representations},
  booktitle = confICLR,
  year = {2020},
}

@article{Ni2024BridgingSA,
  author = {Tianwei Ni and Benjamin Eysenbach and Erfan Seyedsalehi and Michel Ma and Clement Gehring and Aditya Mahajan and Pierre-Luc Bacon},
  title = {Bridging State and History Representations: Understanding Self-Predictive RL},
  journal = {ArXiv},
  volume = {abs/2401.08898},
  year = {2024},
}

@article{Child2020VeryDV,
  author = {Rewon Child},
  title = {Very Deep VAEs Generalize Autoregressive Models and Can Outperform Them on Images},
  journal = {ArXiv},
  volume = {abs/2011.10650},
  year = {2020},
}

@inproceedings{Li2018DisentangledSA,
  author = {Yingzhen Li and Stephan Mandt},
  title = {Disentangled Sequential Autoencoder},
  booktitle = confICML,
  year = {2018},
}

@inproceedings{Johnson2016ComposingGM,
  author = {Matthew J. Johnson and David Kristjanson Duvenaud and Alexander B. Wiltschko and Ryan P. Adams and Sandeep Robert Datta},
  title = {Composing Graphical Models with Neural Networks for Structured Representations and Fast Inference},
  booktitle = confNEU,
  year = {2016},
}

@article{Tishby2015DeepLA,
  author = {Naftali Tishby and Noga Zaslavsky},
  title = {Deep Learning and the Information Bottleneck Principle},
  journal = {2015 IEEE Information Theory Workshop (ITW)},
  pages = {1--5},
  year = {2015},
}

@book{Grunwald2007TheMD,
  author = {Peter D. Gr{\"u}nwald},
  title = {The Minimum Description Length Principle},
  publisher = {Springer},
  year = {2007},
}

@article{koppel1987complexity,
  author = {Moshe Koppel},
  title = {Complexity, Depth, and Sophistication},
  journal = {Complex Systems},
  volume = {1},
  number = {6},
  pages = {1087--1091},
  year = {1987}
}

@article{kolmogorov1974talk,
  author = {A. N. Kolmogorov},
  title = {Talk at the Information Theory Symposium in Tallinn},
  journal = {Estonia (then USSR)},
  year = {1974}
}

@article{antunes2017sophistication,
  author = {Lu{'\i}s Antunes and Bruno Bauwens and Andr{'e} Souto and Andreia Teixeira},
  title = {Sophistication vs Logical Depth},
  journal = {Theory of Computing Systems},
  volume = {60},
  pages = {280--298},
  year = {2017},
  publisher = {Springer}
}

@article{vitanyi2006meaningful,
  title={Meaningful information},
  author={Vit{\'a}nyi, Paul M},
  journal={IEEE Transactions on Information Theory},
  volume={52},
  number={10},
  pages={4617--4626},
  year={2006},
  publisher={IEEE}
}


@incollection{Bennett1988LogicalDepth,
  author = {C. H. Bennett},
  title = {Logical Depth and Physical Complexity},
  booktitle = {The Universal Turing Machine: A Half Century Survey},
  publisher = {Oxford University Press},
  pages = {227--258},
  year = {1988}
}

@techreport{Schmidhuber1997Interesting,
  author = {Schmidhuber, J{\"u}rgen},
  title = {What's Interesting?},
  institution = {IDSIA},
  number = {IDSIA-35-97},
  note = {[ftp://ftp.idsia.ch/pub/juergen/interest.ps.gz](ftp://ftp.idsia.ch/pub/juergen/interest.ps.gz);
    Extended abstract in Proc. Snowbird'98, Utah, 1998; see also \cite{Schmidhuber:02predictable}},
  year = {1997}
}

@inproceedings{schmidhuber1999artificial,
  title={Artificial curiosity based on discovering novel algorithmic predictability through coevolution},
  author={Schmidhuber, J{\"u}rgen},
  booktitle={Proceedings of the 1999 congress on evolutionary computation-cec99 (cat. no. 99th8406)},
  volume={3},
  pages={1612--1618},
  year={1999},
  organization={IEEE}
}

@article{schmidhuber2009simple,
  title={Simple algorithmic theory of subjective beauty, novelty, surprise, interestingness, attention, curiosity, creativity, art, science, music, jokes},
  author={Schmidhuber, J{\"u}rgen},
  journal={Journal of the Society of Instrument and Control Engineers},
  volume={48},
  number={1},
  pages={21--32},
  year={2009},
  publisher={The Society of Instrument and Control Engineers}
}



@article{Zhang2023omni,
  author = {Jenny Zhang and Joel Lehman and Kenneth O. Stanley and Jeff Clune},
  title = {OMNI: Open-endedness via Models of Human Notions of Interestingness},
  journal = {ArXiv},
  volume = {abs/2306.01711},
  year = {2023},
}

